MCMC Variational Inference via Uncorrected Hamiltonian Annealing

Given an unnormalized target distribution we want to obtain approximate samples from it and a tight lower bound on its (log) normalization constant log Z. Annealed Importance Sampling (AIS) with Hamiltonian MCMC is a powerful method that can be used to do this. Its main drawback is that it uses non-differentiable transition kernels, which makes tuning its many parameters hard. We propose a framework to use an AIS-like procedure with Uncorrected Hamiltonian MCMC, called Uncorrected Hamiltonian Annealing. Our method leads to tight and differentiable lower bounds on log Z. We show empirically that our method yields better performances than other competing approaches, and that the ability to tune its parameters using reparameterization gradients may lead to large performance improvements.

==> sections/impact.tex <==
\section{Broader Impact}

Hola.

==> sections/short_version.tex <==
\section{Short Version of Story}

We have the estimator 
\begin{equation}
R(z_1, \rho_1, \hdots, z_M, \rho_M) = \frac{\tilde p(z_M, \rho_M)}{q_w(z_1, \rho_1)} \prod_{m=1}^{M-1} \frac{U_m(z_m, \rho_m\vert z_{m+1}, \rho_{m+1})}{T_m(z_{m+1}, \rho_{m+1}\vert z_m, \rho_m)}. \label{eq:R2}
\end{equation}

\subsection{Hamiltonian AIS}

We need to find a way of defining the forward transitions $T_m(z_{m+1} \rho_{m+1} \vert z_m, \rho_m)$ and the reverse transitions $U_m(z_{m} \rho_{m} \vert z_{m+1} \rho_{m+1})$. Hamiltonian AIS provides one way of doing this. It sets the forward transition $T_m$ to be a Hamiltonian MCMC iteration (leaves $\pi_m(z, \rho) = \pi_m(z) \MD(\rho)$ invariant), and the reverse transition $U_m$ to be the reversal of $T_m$ with respect to $\pi_m(z, \rho)$. Specifically, the processes defining these transitions are given by:
\small\begin{equation}
\left . \begin{array}{l}
T_m(z_{m+1}, \rho_{m+1} \vert z_m, \rho_m): \\
\hspace{0.3cm} 1.\quad \rho' \sim s(\cdot \vert \rho_m)\\
\hspace{0.3cm} 2.\quad (z'', \rho'') = \mathcal{T}_m(z_m, \rho')\\
\hspace{0.3cm} 3.\quad \rho''' = -\rho''\\
\hspace{0.3cm} 4.\quad (z_{m+1}, \rho'''') = \mathrm{AR}((z'', \rho'''), (z_m, \rho'))\\
\hspace{0.3cm} 5.\quad \rho_{m+1} = -\rho'''
\end{array} \right .
\left . \begin{array}{l}
U_m(z_m, \rho_m \vert z_{m+1}, \rho_{m+1}): \\
\hspace{0.3cm} 1.\quad \rho' = -\rho_{m+1}\\
\hspace{0.3cm} 2.\quad (z'', \rho'') = \mathcal{T}_m(z_{m+1}, \rho')\\
\hspace{0.3cm} 3.\quad \rho''' = -\rho''\\
\hspace{0.3cm} 4.\quad (z_{m}, \rho'''') = \mathrm{AR}((z'', \rho'''), (z_{m+1}, \rho'))\\
\hspace{0.3cm} 5.\quad \rho_{m+1} \sim s(\cdot \vert \rho''')\\
\end{array} \right .
\label{eq:TUhais}\end{equation}\normalsize

(I'm thinking maybe do not give this in the main text, but in the appendix? Seems to complicated, and not extremely necessary?)

In order to compute the estimator $R$ from eq.~\ref{eq:R2} we need to compute the ratio $U_m / T_m$. While at a first glance this may appear to be complex, the main advantage of AIS comes from the fact that setting $U_m$ to be the reversal of $T_m$ leads to a simplification. By definition of the reversal of a Markov transition kernel we get that
\begin{equation}
\frac{U_m(z_m, \rho_m \vert z_{m+1}, \rho_{m+1})}{T_m(z_{m+1}, \rho_{m+1} \vert z_m, \rho_m)} = \frac{\tilde \pi_m(z_{m+1}, \rho_{m+1})}{\tilde \pi_m(z_m, \rho_m)},
\end{equation}
and thus the estimator $R$ from eq.~\ref{eq:R2} becomes
\begin{equation}
R(z_1, \rho_1, \hdots, z_M, \rho_M) = \frac{\tilde p(z_M, \rho_M)}{q_w(z_1, \rho_1)} \prod_{m=1}^{M-1} \frac{\tilde \pi_m(z_m, \rho_m)}{\tilde \pi_m(z_{m+1}, \rho_{m+1})}.
\end{equation}
Using $\tilde p(z, \rho) = \tilde p(z) \MD(\rho)$, $q_w(z, \rho) = q_w(z) \MD(\rho)$ and $\tilde \pi_m(z, \rho) = \tilde \pi_m(z) \MD(\rho)$ we get
\begin{equation}
R(z_1, \rho_1, \hdots, z_M, \rho_M) = \frac{\tilde p(z_M)}{q_w(z_1)} \prod_{m=1}^{M-1} \frac{\tilde \pi_m(z_m)}{\tilde \pi_m(z_{m+1})}.
\end{equation}

\subsection{Uncorrected Hamiltonian AIS}

We propose Uncorrected Hamiltonian AIS, which uses the transitions from eq.~\ref{eq:TUuhais}
\small\begin{equation}
\left . \begin{array}{l}
T_m(z_{m+1}, \rho_{m+1} \vert z_m, \rho_m): \\
\hspace{0.3cm} 1.\quad \rho' \sim s(\cdot \vert \rho_m)\\
\hspace{0.3cm} 2.\quad (z_{m+1}, \rho_{m+1}) = \mathcal{T}_m(z_m, \rho')\\
\end{array} \right .
\left . \begin{array}{l}
U_m(z_m, \rho_m \vert z_{m+1}, \rho_{m+1}): \\
\hspace{0.3cm} 1.\quad \rho' = -\rho_{m+1}\\
\hspace{0.3cm} 2.\quad (z_m, \rho'') = \mathcal{T}_m(z_{m+1}, \rho')\\
\hspace{0.3cm} 3.\quad \rho''' = -\rho''\\
\hspace{0.3cm} 4.\quad \rho_{m+1} \sim s(\cdot \vert \rho''')\\
\end{array} \right .
\label{eq:TUuhais}\end{equation}\normalsize
These are just the transitions from eq.~\ref{eq:TUhais} without the accept/reject step.

\textbf{Note:} Since $\mathcal{T}^{-1}$ is just negating the momentum, running $\mathcal{T}_m$, and negating the momentum again, the transitions from eq.~\ref{eq:TUuhais} can be written as (which I think is way nicer, but requires more of an explanation -- But I think I'd use these, the explanation is only about the inverse which is ok I guess, just a few lines)
\small\begin{equation}
\left . \begin{array}{l}
T_m(z_{m+1}, \rho_{m+1} \vert z_m, \rho_m): \\
\hspace{0.3cm} 1.\quad \rho_{m+1/2} \sim s(\cdot \vert \rho_m)\\
\hspace{0.3cm} 2.\quad (z_{m+1}, \rho_{m+1}) = \mathcal{T}_m(z_m, \rho_{m+1/2})\\
\end{array} \right .
\left . \begin{array}{l}
U_m(z_m, \rho_m \vert z_{m+1}, \rho_{m+1}): \\
\hspace{0.3cm} 1.\quad (z_m, \rho_{m+1/2}) = \mathcal{T}^{-1}_m(z_{m+1}, \rho_{m+1})\\
\hspace{0.3cm} 2.\quad \rho_{m} \sim s(\cdot \vert \rho_{m+1/2})\\
\end{array} \right .
\label{eq:TUuhais2}\end{equation}\normalsize
For these choices for $T_m$ and $U_m$ the ratio $U_m / T_m$ takes the form
\small\begin{equation}
\frac{U_m(z_m, \rho_m \vert z_{m+1}, \rho_{m+1})}{T_m(z_{m+1}, \rho_{m+1} \vert z_m, \rho_m)} = \frac{s(\rho_m\vert \rho_{m+1/2})}{s(\rho_{m+1/2}\vert \rho_m)}
, \quad \mbox{ and } \quad R = \frac{\tilde p(z_M) \MD(\rho_M)}{q_w(z_1) \MD(\rho_1)} \prod_{m = 1}^{M - 1} \frac{s(\rho_m\vert \rho_{m+1/2})}{s(\rho_{m+1/2}\vert \rho_m)}. \label{eq:R2first}
\end{equation}\normalsize
If, in addition, we consider a re-sampling distribution $s(\rho\vert \rho')$ that satisfies detailed balance with respect to $\MD(\rho)$ (satisfied by full and partial re-sampling), we can further simplify the expressions to
\small\begin{equation}
\frac{U_m(z_m, \rho_m \vert z_{m+1}, \rho_{m+1})}{T_m(z_{m+1}, \rho_{m+1} \vert z_m, \rho_m)} = \frac{\MD(\rho_m)}{\MD(\rho_{m+1/2})}
, \quad \mbox{ and } \quad R_2 = \frac{\tilde p(z_M)}{q_w(z_1)} \prod_{m = 1}^{M - 1} \frac{\MD(\rho_{m+1})}{\MD(\rho_{m+1/2})}. \label{eq:R2simple}
\end{equation}\normalsize



